Solutions of Polynomial Systems Derived from the Steady Cavity Flow Problem

We propose a general algorithm to enumerate all solutions of a zero-dimensional polynomial system with respect to a given cost function. The algorithm is developed and is used to study a polynomial system obtained by discretizing the steady cavity flow problem in two dimensions. The key technique on which our algorithm is based is to solve polynomial optimization problems via sparse semidefinite programming relaxations (SDPR), which has been adopted successfully to solve reaction-diffusion boundary value problems recently. The cost function to be minimized is derived from discretizing the fluid's kinetic energy. The enumeration algorithm's solutions are shown to converge to the minimal kinetic energy solutions for SDPR of increasing order. We demonstrate the algorithm with SDPR of first and second order on polynomial systems for different scenarios of the cavity flow problem and succeed in deriving the $k$ smallest kinetic energy solutions. The question whether these solutions converge to solutions of the steady cavity flow problem is discussed, and we pose a conjecture for the minimal energy solution for increasing Reynolds number.

==> Fig/44point.tex <==
%WinTpicVersion3.08
\unitlength 0.1in
\begin{picture}( 13.0700, 13.0300)( 13.8900,-21.0300)
% BOX 2 0 3 0
% 2 1400 800 2696 2103
% 
\special{pn 8}%
\special{pa 1400 800}%
\special{pa 2696 800}%
\special{pa 2696 2104}%
\special{pa 1400 2104}%
\special{pa 1400 800}%
\special{fp}%
% LINE 2 0 3 0
% 6 1400 1232 2696 1232 1400 1671 2696 1671 1839 800 1839 2103
% 
\special{pn 8}%
\special{pa 1400 1232}%
\special{pa 2696 1232}%
\special{fp}%
\special{pa 1400 1672}%
\special{pa 2696 1672}%
\special{fp}%
\special{pa 1840 800}%
\special{pa 1840 2104}%
\special{fp}%
% LINE 2 0 3 0
% 2 2271 800 2271 2103
% 
\special{pn 8}%
\special{pa 2272 800}%
\special{pa 2272 2104}%
\special{fp}%
% STR 2 0 3 0
% 3 1839 1599 1839 1671 4 0
% (1,1)
\put(18.3900,-16.7100){\makebox(0,0)[rt]{(1,1)}}%
% STR 2 0 3 0
% 3 2271 1599 2271 1671 1 0
% (2,1)
\put(22.7100,-16.7100){\makebox(0,0)[lt]{(2,1)}}%
% STR 2 0 3 0
% 3 1839 1160 1839 1232 3 0
% (1,2)
\put(18.3900,-12.3200){\makebox(0,0)[rb]{(1,2)}}%
% STR 2 0 3 0
% 3 2271 1160 2271 1232 2 0
% (2,2)
\put(22.7100,-12.3200){\makebox(0,0)[lb]{(2,2)}}%
% DOT 0 0 3 0
% 5 1841 1232 1841 1673 2273 1673 2273 1232 2273 1232
% 
\special{pn 20}%
\special{sh 1}%
\special{ar 1842 1232 10 10 0  6.28318530717959E+0000}%
\special{sh 1}%
\special{ar 1842 1674 10 10 0  6.28318530717959E+0000}%
\special{sh 1}%
\special{ar 2274 1674 10 10 0  6.28318530717959E+0000}%
\special{sh 1}%
\special{ar 2274 1232 10 10 0  6.28318530717959E+0000}%
\special{sh 1}%
\special{ar 2274 1232 10 10 0  6.28318530717959E+0000}%
\end{picture}%

